On the Effectiveness of Lipschitz-Driven Rehearsal in Continual Learning

Rehearsal approaches enjoy immense popularity with Continual Learning (CL) practitioners. These methods collect samples from previously encountered data distributions in a small memory buffer; subsequently, they repeatedly optimize on the latter to prevent catastrophic forgetting. This work draws attention to a hidden pitfall of this widespread practice: repeated optimization on a small pool of data inevitably leads to tight and unstable decision boundaries, which are a major hindrance to generalization. To address this issue, we propose Lipschitz-DrivEn Rehearsal (LiDER), a surrogate objective that induces smoothness in the backbone network by constraining its layer-wise Lipschitz constants w.r.t. replay examples. By means of extensive experiments, we show that applying LiDER delivers a stable performance gain to several state-of-the-art rehearsal CL methods across multiple datasets, both in the presence and absence of pre-training. Through additional ablative experiments, we highlight peculiar aspects of buffer overfitting in CL and better characterize the effect produced by LiDER. Code is available at https://github.com/aimagelab/LiDER

==> contents/8_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
\begin{comment}

The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit. In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.

\end{comment}
%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{} 
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{} The code for reproducing our experiments can be found in the supplemental material and will be made publicly available at publication.
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{} We cover these aspects in the main paper (Sec.~\ref{sec:experiments}) and, more in depth, in the supplemental materials.
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{} Due to space constraints, variance values for our experiments are included in the supplemental material.
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNo{} Experiments were conducted on an on-premise desktop machine, equipped with a RTX 2080 consumer GPU. However, we did not keep a detailed record of total computation time.
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{} In our work we use original code, with the only exceptions for the evaluation datasets whose original papers are cited.
  \item Did you mention the license of the assets?
    \answerNA{} Our work uses original code and freely available datasets.
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{} We use datasets commonly established and used in literature, for which, to the best of our knowledge, the issues mentioned above have never been found to affect them.
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> contents/tables/results_variances.tex <==
\begin{table}[t]
\begin{center}
\caption{Standard errors for the comparative evaluation reported in the main paper.}
\label{table:var}
\rowcolors{4}{lightgray}{}
\begin{tabular}{l@{\hskip 0.5cm}cc@{\hskip 0.5cm}cc@{\hskip 0.5cm}cc@{\hskip 0.5cm}cc}
\hline\noalign{\smallskip}
\textbf{Benchmark} & \multicolumn{4}{c}{\textbf{\small{Split CIFAR-100}}} & \multicolumn{2}{c@{\hskip 0.5cm}}{\textbf{\small{Split \miniimagenet}}} & \multicolumn{2}{c@{\hskip 0.5cm}}{\textbf{\small{Split CUB-200}}}\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\textbf{Pre-training} & \multicolumn{2}{c@{\hskip 0.5cm}}{\xmark} & \multicolumn{2}{c@{\hskip 0.5cm}}{\textit{Tiny ImageNet}} & \multicolumn{2}{c@{\hskip 0.5cm}}{\xmark} & \multicolumn{2}{c@{\hskip 0.5cm}}{\textit{ImageNet}}\\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
Joint    (UB)    & \multicolumn{2}{c}{\var{0.61}} & \multicolumn{2}{c}{\var{0.49}} & \multicolumn{2}{c}{\var{0.85}} & \multicolumn{2}{c}{\var{0.45}} \\
\rowcolor{lightgray}
Finetune         & \multicolumn{2}{c}{\var{0.15}} & \multicolumn{2}{c}{\var{0.24}} & \multicolumn{2}{c}{\var{0.03}} & \multicolumn{2}{c}{\var{0.09}} \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
\rowcolor{white}
\textbf{Buffer Size} & $500$ & $2000$ & $500$ & $2000$ & $2000$ & $5000$ & $400$ & $1000$ \\
\noalign{\smallskip}
\hline
\noalign{\smallskip}
iCaRL~\cite{rebuffi2017icarl} & \var{0.56} & \var{0.34}   & \var{0.36}  & \var{0.33} & \var{0.25} & \var{0.71}   & \var{0.56} & \var{0.52} \\
\hspace{.3em} + LiDER         & \var{0.32} & \var{0.64} & \var{0.48} & \var{0.09} 	& \var{0.14} & \var{0.47} & \var{0.06} & \var{0.02} \\
\dpp~\cite{buzzega2020dark}  & \var{0.74} & \var{1.50}   & \var{1.80}  & \var{1.12} 	& \var{0.37} & \var{0.74}   & \var{1.40} & \var{1.16} \\
\hspace{.3em} + LiDER                  & \var{1.11}   & \var{1.61}   & \var{0.67} & \var{1.91} 	& \var{1.07} & \var{0.78}   & \var{0.24} & \var{1.39} \\
GDumb~\cite{prabhu2020gdumb} & \var{1.81}  & \var{1.25}   & \var{1.74}  & \var{1.49} 	& \var{1.51}   & \var{0.95}   & \var{1.09} & \var{1.28} \\
\hspace{.3em} + LiDER        & \var{0.86}   & \var{0.64}   & \var{0.23}   & \var{0.40} 	& \var{0.70} & \var{0.51} & \var{0.15} & \var{0.21} \\
ER-ACE~\cite{caccia2022new} & \var{0.45} & \var{1.04} & \var{0.64} & \var{0.73} 	& \var{1.21}   & \var{0.66}   & \var{0.40} & \var{0.75} \\
\hspace{.3em} + LiDER       & \var{0.33}   & \var{0.71}   & \var{0.24}   & \var{0.19} 	& \var{0.58} & \var{0.17} & \var{0.51}  & \var{0.04} \\
\hline
\end{tabular}
\end{center}
\end{table}
